Recursive relations in the cohomology rings of moduli spaces of rank 2 parabolic bundles on the Riemann sphere

We study the singular cohomology of the moduli space of rank 2 parabolic bundles on a Riemann surface where the weights are all 1/4. We give a formula, based on work of Boden, for the Poincar\'e polynomial of this moduli space in general, and deduce a complete set of relations in the cohomology ring for the case when the genus is zero. These relations are recursive in the number of parabolic points (which must be odd), and are analogous to the relations appearing in the cohomology ring for the non-parabolic story, which are recursive in the genus. Our methods use techniques from a paper of Weitsman to reduce to a linear algebra problem, which we then solve using the theory of orthogonal polynomials and a continued fraction expansion for the generating function of the Euler numbers.

==> bibliography.tex <==
% ----------------------------------------------------------------

% the page number on the first page of the bibliography has to be
% centered at the bottom (!)

\thispagestyle{plain}

% the bibliography has to be single-spaced within items but
% double-spaced between items

\let\oldthebibliography=\thebibliography
\let\endoldthebibliography=\endthebibliography
\renewenvironment{thebibliography}[1]{
  \begin{oldthebibliography}{#1}
    \setlength{\itemsep}{3ex}
  }{
    \end{oldthebibliography}
  }

\bibliographystyle{abbrv}
\bibliography{biblio}


\begin{thebibliography}{1}

\bibitem{don1} S. K. Donaldson, \emph{Symplectic Submanifolds and Almost-Complex Geometry}, 
J. Differential Geom. \textbf{44} (1996) 666-705.
\bibitem{nitsure_cohom} a
\bibitem{boden_parabolic} b
\bibitem{weitsman_cohom} c
\bibitem{weitsman_toric_I} d
\bibitem{AB} e
\bibitem{biswas_cohom} f
\bibitem{kirk_klassen} g
\bibitem{munoz_cohom} h
\bibitem{salamon_dostoglou} i
\bibitem{donaldson_kron} p
\bibitem{kron_mrowka_knot_instanton} j
\bibitem{kron_mrowka_uknot} k 
\bibitem{kron_mrowka_sutures} l
\bibitem{kron_mrowka_embedded} m
\bibitem{kron_mrowka_alexander} q
\bibitem{siebert_tian} n

\end{thebibliography}

% ----------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

% ----------------------------------------------------------------
